Real World Application of Quantum-Classical Optimization for Production Scheduling

This work is a benchmark study for quantum-classical computing method with a real-world optimization problem from industry. The problem involves scheduling and balancing jobs on different machines, with a non-linear objective function. We first present the motivation and the problem description, along with different modeling techniques for classical and quantum computing. The modeling for classical solvers has been done as a mixed-integer convex program, while for the quantum-classical solver we model the problem as a binary quadratic program, which is best suited to the D-Wave Leap's Hybrid Solver. This ensures that all the solvers we use are fetched with dedicated and most suitable model(s). Henceforth, we carry out benchmarking and comparisons between classical and quantum-classical methods, on problem sizes ranging till approximately 150000 variables. We utilize an industry grade classical solver and compare its results with D-Wave Leap's Hybrid Solver. The results we obtain from D-Wave are highly competitive and sometimes offer speedups, compared to the classical solver.

==> sections/2_4_qubo.tex <==
\subsection{Quantum Model: Quadratic Unconstrained Binary Optimization}~\label{sec:qubo}

A quadratic unconstrained binary optimization (QUBO) problem is problem of the following kind:
\begin{equation}
\text{minimize} \{ x^TQx : x \text{ binary} \} .
\end{equation}
QUBOs are a natural representation for problems that can be solved using quantum annealing, as the objective function is quadratic, which aligns well with the energy landscape of the physical system being simulated. Many real-world optimization problems can be formulated as QUBO instances.

To convert our binary quadratic problems, which can be written as
\begin{equation}
\text{minimize} \{ x^TQx : x \in X, x \text{ binary} \}.
\end{equation}
for the feasible set $X$, into a QUBO, we need to transform the constraints into an objective.

That each job $j \in \mathcal{J}$ is scheduled exactly once is ensured by
\begin{equation}
\sum_{m \in \mathcal{M}}\sum_{t \in \mathcal{T}}x_{m,t,j} = 1.
\end{equation}
This equation holds for an $x$ if and only if
\begin{equation}
\left( \sum_{m \in \mathcal{M}}\sum_{t \in \mathcal{T}} x_{m,t,j} - 1\right)^2 = 0.
\end{equation}
That is, $x$ minimizes the left hand side. 

The constraints that ensures that maximum one job can be processed on a machine $m \in \mathcal{M}$ at any time $t\in \mathcal{T}$
\begin{equation}
\sum_{j \in \mathcal{J}} x_{m,t,j} \leq 1.
\end{equation}
is fulfilled if and only if
\begin{equation}
\sum_{i \in \mathcal{J}} \sum_{j \in \mathcal{J} \setminus \{i\}} x_{m,t,i} x_{m,t,j} = 0.
\end{equation}
Again, if the left hand side is zero, $x$ minimizes the left hand side.

Because 
\begin{equation}
\sum_{j \in \mathcal{J}} x_{m,t,j} \in \{0,1\}
\end{equation}
is ensured for all machines $m \in \mathcal{M}$ and times $t \in \mathcal{T}$, the inequality
\begin{equation}
\sum_{j \in \mathcal{J}} x_{m,t,j} \leq \sum_{j \in \mathcal{J}} x_{m,t-1,j}.
\end{equation}
if fulfilled if and only if
\begin{equation}
\left(\sum_{j \in \mathcal{J}} x_{m,t,j}\right) \left(\sum_{j \in \mathcal{J}} x_{m,t,j} - \sum_{j \in \mathcal{J}} x_{m,t-1,j}\right) = 0,
\end{equation}
i.e., the left hand side is minimal.

Combining the minimization problems derived from the constraint with the original objective we get the QUBO
\begin{align}
 &\text{minimize} \\
 & \sum_{m \in \mathcal{M}} \sum_{t \in \mathcal{T}_2} \sum_{i \in \mathcal{J}} \sum_{j \in \mathcal{J}} s_{i,j}x_{m,t-1,i}x_{m,t,j} \\
+ & \sum_{m \in \mathcal{M}} \left( \sum_{t \in \mathcal{T}} \sum_{j \in \mathcal{J}} p_j x_{m,t,j}\right)^2 \\
- & \sum_{m \in \mathcal{M}} \sum_{i \in \mathcal{J}_0} \sum_{j \in \mathcal{J}} c_{m,j} x_{m,i,j} \\
+ \lambda_1 & \sum_{j \in \mathcal{J}} \left( \sum_{m \in \mathcal{M}}\sum_{t \in \mathcal{T}} x_{m,t,j} - 1\right)^2 \\
+ \lambda_2 & \sum_{m \in \mathcal{M}}\sum_{t \in \mathcal{T}} \sum_{i \in \mathcal{J}} \sum_{j \in \mathcal{J} \setminus \{i\}} x_{m,t,i} x_{m,t,j} \\
+ \lambda_3 & \sum_{m \in \mathcal{M}}\sum_{t \in \mathcal{T}} \left( \sum_{j \in \mathcal{J}} x_{m,t,j} \right) \left(\sum_{j \in \mathcal{J}} x_{m,t,j} - \sum_{j \in \mathcal{J}} x_{m,t-1,j}\right)
\end{align}
that is equivalent to the previous optimization problems for big enough $\lambda_1, \lambda_2, \lambda_3$. 

The parameters have to be chosen such that violating a constraint adds more to the overall objective than the possible gains in the original objective. In addition, we need to pay attention to the part of the objective that corresponds to the constraints that ensures that the solution is a sequence of jobs on each machine, which only holds if at most one job is scheduled on each machine at any time. 

If violating the ordering constraints the benefit in the objective is that it saves setup times. Therefore, we can choose 
\begin{equation}
\lambda_3 = \text{maximum} \{ s_{i,j} : i,j \in \mathcal{J} \} + 1.
\end{equation}

When not choosing a job, one can save the setup times, hence 
\begin{equation}
\lambda_1 > \text{maximum} \{ s_{i,j} : i,j \in \mathcal{J} \} =: s^*.
\end{equation}
Also, not choosing a job can reduce the balancing objective. It is clear that not choosing the job $k \in \mathcal{J}$ with the highest processing time is the most beneficial. Due to the convexity of the balancing part of the objective, the most can be gained when all jobs are allocated to one machine. We now compute how much we can save the most when not selecting job $k$. From 
\begin{align}
\left( \sum_{j \in \mathcal{J}} p_j \right)^2 &= \left( \sum_{j \in \mathcal{J} \setminus \{k\} } p_j + p_k \right)^2 \\
&= \left( \sum_{j \in \mathcal{J} \setminus \{k\}} p_j \right)^2 + 2 \left( \sum_{j \in \mathcal{J} \setminus \{k\}} p_j \right)^2 p_k + p_k^2 \\
&\leq \left( \sum_{j \in \mathcal{J} \setminus \{k\}} p_j \right)^2 2 (J-1)p_k^2 + 2 p_k^2 \\
&= 2 J p_k^2
\end{align}
follows, that not selecting job $k$ can decrease the objective by at most $2 J p_k^2$. Hence,
\begin{equation}
\lambda_1 > 2 J p_k^2.
\end{equation}
Selecting more than one job increases the value create by the job. Therefore,
\begin{equation}
\lambda_1 > \text{maximum} \{ c_{m,j} : m \in \mathcal{M}, j \in \mathcal{J} \} 0: c^*.
\end{equation}
For $\lambda_1$ we get
\begin{equation}
\lambda_1 = \text{maximum}(s^*, 2 J p_k^2, c^*) +1 .
\end{equation}













==> sections/2_5_decomposition.tex <==
\subsection{decomposition}

The decomposition technique divides the problem into two subproblems based on the machines. We create a graph where each machine is represented by a node. An edge exists between two nodes, with the edge's weight corresponding to the number of jobs that can be performed on both machines.

The Kernighan-Lin algorithm can be used to find the minimum cut that divides this graph into two subgraphs with the same amount of nodes. The runtime is \( O(n^2 \log n) \). Now we need to decide which jobs should be assigned to which subproblem. To simplify this process, we determine for each job on which machine it has the highest job value. The job is then assigned to the subproblem that includes that machine.

This process can be iteratively repeated until an appropriate size for the problem is reached or if the number of machines in the subproblems is smaller than 4. Note that the whole solutions created by the solutions of the subproblems is always feasible, but not always optimal, even if the solutions of the subproblems are optimal.

==> sections/2_X_saves.tex <==

\begin{itemize}
    \item \aanote{} Problem Description 
    \item \fknote{} Classical Model: Convex IP version
    \item \aanote{} QUBO Formulation (for QPU and BQM Solver) 
    \item \aanote{} CQM Modeling (0-1 IP formulation) 
\end{itemize}

\subsection{Classical Model: 0/1 Quadratic Integer Programming}

Define a binary variable $x_{j,m}^{n}$ such that

\begin{equation*}
x_{j,m}^{n} = \begin{cases}
1, &\text{if job $j$ is the $n$th job processed by machine $m$} \;,\\
0, &\text{otherwise}\;.
\end{cases}
\end{equation*}
With $j \in \mathcal{J}, m \in {E_j}$ and $n \in (0, |P_{m}|)$ where $|P_{m}|$ is the cardinality of the set containing the possible jobs for machine m. 


\subsection{Constraints}
\subsubsection{Constraint 1: Only eligible machines can process a job}\label{sec:cons:cons1}
As a numerical penalty on our QUBO, the expression for this constraint is given by equation below. However, the way in which we defined our binary variables takes care of this constraint by removing all the variables that violate it. 
\begin{align*}
    \text{Constant Bits: }x_{j,m}^n=0, \forall j, \forall m \notin {E_j},  \forall n \;.
\end{align*}


\subsubsection{Constraint 2: Maximum one job can be processed by a machine at any time}

\begin{equation*}
    \sum_{\forall j}  x_{j,m}^n \leq 1, \forall n,  \forall m\;.
\end{equation*}

\subsubsection{Constraint 3: On any machine a job can be processed at $(n+1)$th sequence iff a job was processed at the $n$th sequence}

\begin{equation*}
    \sum_{\forall j}  x_{j,m}^{n+1} \leq \sum_{\forall j}  x_{j,m}^n \;, \forall n,  \forall m\;.
\end{equation*}


\subsubsection{Constraint 4: All the jobs must be processed by some machine at some sequence}

\begin{equation*}
    \sum_{\forall m} \sum_{\forall n} x_{j,m}^{n} = 1, \forall j\;.
\end{equation*}

\subsection{Objectives}
\subsubsection{Maximize job values}

\begin{equation}
    \alpha \cdot \max \sum_{\forall m}  \sum_{\forall j} \sum_{\forall n} v_j^m \cdot x_{j,m}^n
\end{equation}

\subsubsection{Minimize set-up times}

\begin{equation}
    \min \sum_{\forall j}\sum_{\forall j'}\sum_{\forall n} \sum_{\forall m} s_{j,j'}\cdot x_{j,m}^n \cdot x_{j',m}^{n+1}
\end{equation}


\subsubsection{Uniform busy times of machines}
\begin{equation}
    \min \sum_{\forall m}\left(\sum_{\forall j} \sum_{\forall n} p_j \cdot x_{j,m}^n \right)^2 \;.
\end{equation}

\subsection{QUBO Formulation}
\aanote{need to combine this with Classical Model: 0/1 Quadratic Integer Programming, and present it as a table}
Define a binary variable $x_{j,m}^{n}$ such that

\begin{equation*}
x_{j,m}^{n} = \begin{cases}
1, &\text{if job $j$ is the $n$th job processed by machine $m$} \;,\\
0, &\text{otherwise}\;.
\end{cases}
\end{equation*}
With $j \in \mathcal{J}, m \in {E_j}$ and $n \in (0, |P_{m}|)$ where $|P_{m}|$ is the cardinality of the set containing the possible jobs for machine m. 


\subsection{Constraints}
\subsubsection{Constraint 1: Only eligible machines can process a job}
As a numerical penalty on our QUBO, the expression for this constraint is given by equation below. However, the way in which we defined our binary variables takes care of this constraint by removing all the variables that violate it. 
\begin{align*}
    \text{Constant Bits: }x_{j,m}^n=0, \forall j, \forall m \notin {E_j},  \forall n \;.
\end{align*}


\subsubsection{Constraint 2: Maximum one job can be processed by a machine at any time}

\begin{equation}
    \lambda_3 \cdot \sum_{\forall n} \sum_{\forall  m}\left(\sum_{\forall j}  x_{j,m}^n \right)\cdot \left(\sum_{\forall j}  x_{j,m}^n -1 \right) \;.
\end{equation}

\begin{equation*}
    \lambda_3 = \alpha \cdot \max(\text{job values}) + 2 \cdot \max(\text{set-up times}) + \lambda_4
\end{equation*}

\subsubsection{Constraint 3: On any machine a job can be processed at $(n+1)$th sequence iff a job was processed at the $n$th sequence}

\begin{equation}
    \lambda_4 \cdot \sum_{\forall n} \sum_{\forall  m} \left(1- \sum_{\forall j}  x_{j,m}^n \right)\cdot \left(\sum_{\forall j}  x_{j,m}^{n+1} \right) \;.
\end{equation}

\begin{equation*}
    \lambda_4 = \alpha \cdot \max(\text{job values}) + \max(\text{set-up times})
\end{equation*}

\subsubsection{Constraint 4: All the jobs must be processed by some machine at some sequence}

\begin{equation}
    \lambda_5 \cdot  \sum_{\forall j} \left(\sum_{\forall m} \sum_{\forall n} x_{j,m}^{n}-1\right)^2 \;.
\end{equation}

\begin{equation*}
    \lambda_5 = \alpha \cdot \max(\text{job values}) + \max(\text{set-up times})
\end{equation*}

\subsection{Objectives}
\subsubsection{Maximize job values}

\begin{equation}
    \alpha \cdot \max \sum_{\forall m}  \sum_{\forall j} \sum_{\forall n} v_j^m \cdot x_{j,m}^n
\end{equation}

\subsubsection{Minimize set-up times}

\begin{equation}
    \min \sum_{\forall j}\sum_{\forall j'}\sum_{\forall n} \sum_{\forall m} s_{j,j'}\cdot x_{j,m}^n \cdot x_{j',m}^{n+1}
\end{equation}


\subsubsection{Uniform busy times of machines}
\begin{equation}
    \min \sum_{\forall m}\left(\sum_{\forall j} \sum_{\forall n} p_j \cdot x_{j,m}^n \right)^2 \;.
\end{equation}





==> sections/3_methods_algorithms.tex <==


\section{Optimization Solvers}~\label{sec:methods}

\subsection{Gurobi Solver}
Gurobi is a powerful mathematical programming solver that utilizes the branch and bound algorithm. It is considered state-of-the-art and is designed to run on classical hardware. This algorithm works by breaking down the original problem into smaller sub-problems using a decision tree. By using lower bounds derived from linear programming relaxations, Gurobi is able to reduce the search space and improve efficiency~\cite{gurobi}.

\begin{figure*}[t]
\centering
\begin{minipage}{1\columnwidth}
\centering
\includegraphics[width=\textwidth]{figures/1_FINAL_SOLUTIONS.pdf}
\caption{\small{Final objective value obtained from the two solvers, for different problem sizes. The plots show that the solution quality is almost identical.}}
\label{fig1}
\end{minipage}%
\quad
\begin{minipage}{1\columnwidth}
\centering
\includegraphics[width=0.98\textwidth]{figures/2_Percentage_Deviation_Full.pdf}
\caption{\small{Percentage deviation of DWave CQM solvers final objective value, from the final solution of Gurobi. We can see that the worst solution provided by DWave is within $2.6\%$ to that of Gurobi solver.}}
\label{fig2}
\end{minipage}
\end{figure*}

Gurobi is an all-purpose solver, meaning it can be used to solve a wide range of optimization problems. It is capable of finding a guaranteed optimal solution in a deterministic manner, given enough time. In the context of this work, the cloud-based service of Gurobi solver was utilized. It ran on an Intel(R) Xeon(R) Platinum 8124M CPU, which has a clock speed of 3.00 GHz and 8 physical cores. This combination of hardware and software provides a powerful and reliable optimization solution.



\subsection{DWave's CQM Solver}
DWave provides quantum as well hybrid solvers to solve optimization problems. It provides several quantum annealers via cloud-based access, which have over $5000$ qubits and an average of $15$ couplers per qubit \cite{farre}. These quantum computers are designed to solve Quadratic Unconstrained Binary Optimization (QUBO) problems. In a QUBO problem, each optimization variable is represented by a qubit, and the optimal solution corresponds to the ground state of the system. The quantum annealing mechanism employed by D-Wave aims to find the ground state by evolving the quantum system over time and then measuring all the qubits to reveal the optimal solution. 



However, D-Wave's hardware has limited connectivity, meaning that each qubit can only interact with a certain number of other qubits. This limitation imposes constraints on the correlations that can be represented by the Hamiltonian encoding the QUBO problem. Additionally, finding a suitable representation of the problem with these connectivity constraints is a computationally challenging task known as an NP-hard problem. To overcome this challenge, D-Wave's CQM solver utilized both classical and quantum hardware.

The CQM solver allows for the solution of larger optimization problems that exceed the capacity of the quantum hardware by decomposing the original problem into smaller parts and presenting only a subset of the problem to the quantum annealer. However, the exact workings of CQM are not publicly disclosed.

\begin{table}[!htbp]
\centering
\begin{tabular}{c|c|c|c|c|c} \hline\hline
\multirow{2}{*}{\textbf{Id}} & \multirow{2}{*}{\textbf{Jobs}} & \multirow{2}{*}{\textbf{Machines}} & \textbf{D-Wave} & \textbf{Gurobi} & \textbf{D-Wave} \\ 
& & & \textbf{Variables} & \textbf{Variables} & \textbf{Runtime (seconds)} \\ \hline 
1 & 27 & 9 & 2012 & 2432 & 5.00 \\ \hline
2 & 27 & 9 & 2092 & 2518 & 5.00 \\ \hline
3 & 45 & 9 & 4905 & 5550 & 7.39 \\ \hline
4 & 48 & 8 & 5065 & 5684 & 8.48 \\ \hline
5 & 50 & 10 & 9507 & 10448 & 23.52 \\ \hline
6 & 60 & 10 & 10211 & 11182 & 27.71 \\ \hline
7 & 60 & 15 & 11897 & 13184 & 25.68 \\ \hline
8 & 63 & 9 & 12310 & 13324 & 42.32 \\ \hline
9 & 63 & 9 & 12379 & 13396 & 42.75 \\ \hline
10 & 63 & 9 & 12616 & 13642 & 44.40 \\ \hline
11 & 72 & 9 & 12620 & 13640 & 46.59 \\ \hline
12 & 60 & 15 & 12695 & 14024 & 29.06 \\ \hline
13 & 75 & 15 & 20119 & 21790 & 68.89 \\ \hline
14 & 60 & 20 & 20414 & 22362 & 54.24 \\ \hline
15 & 60 & 20 & 21341 & 23334 & 58.70 \\ \hline
16 & 90 & 15 & 28056 & 30024 & 131.66 \\ \hline
17 & 80 & 20 & 31585 & 33998 & 127.22 \\ \hline
18 & 80 & 20 & 33202 & 35672 & 140.50 \\ \hline
19 & 100 & 20 & 47732 & 50694 & 281.87 \\ \hline
20 & 160 & 20 & 151556 & 156810 & 2744.98 \\ \hline \hline
\end{tabular}
\caption{Problem instances used for benchmarking in this work. Gurobi was provided with a constant runtime of three hours.}
\label{table_1}
\end{table}

% \textbf{Quantum Annealing}
% Quantum annealing is specified by two Hamiltonians $H_0$ and $H_1$ acting on $n$ particles \cite{Albash_2018}. The first Hamiltonian is given by $H_0 = \sum_i^n \sigma^x_i$, where $\sigma^x$ is the representation of the Pauli matrix X. Since the system always strives for its lowest energy state, all qubits will be in superposition, as this is the eigenvector with the lowest eigenvalue for this Hamiltonian. The second Hamiltonian $H_1 = \sum_{i}^n h_i\sigma^z_i + \sum_{i, j}^n J_{i,j} \sigma^z_i \sigma^z_i $ denotes the problem formulation as an Ising model. $\sigma^z$ are the representations of the Pauli Z matrices. The parameter $t \in [0,1]$ represents the time:

% \begin{align}\label{Adiabatic Hamiltonian}
% H(t) = (1-t)H_0(t) + tH_1(t)
% \end{align}

% The adiabatic theorem shows, that the system remains in the ground state and thus solves the computational problem if it is sufficiently slow. The maximum runtime can be stated by $\frac{|ln(g)|^{6\alpha}}{g^2}$, where g is the minimum energy gap between the ground state and the first excited state \cite{Elgart_2012}. However, the noise of current quantum annealing systems leads to random bit flips and thus results are not always optimal, even with sufficiently slow annealing processes.

% See \cite{leibl} for a similar discussion for the Gurobi and the D-Wave's Leap framework.



